Ultrafast Hot-Carrier Dynamics in Ultrathin Monocrystalline Gold

Applications in photodetection, photochemistry, and active metamaterials and metasurfaces require fundamental understanding of ultrafast nonthermal and thermal electron processes in metallic nanosystems. Significant progress has been recently achieved in synthesis and investigation of low-loss monocrystalline gold, opening up opportunities for its use in ultrathin nanophotonic architectures. Here, we reveal fundamental differences in hot-electron thermalisation dynamics between monocrystalline and polycrystalline ultrathin (down to 10 nm thickness) gold films. Comparison of weak and strong excitation regimes showcases a counterintuitive unique interplay between thermalised and non-thermalised electron dynamics in mesoscopic gold with the important influence of the X-point interband transitions on the intraband electron relaxation. We also experimentally demonstrate the effect of hot-electron transfer into a substrate and the substrate thermal properties on electron-electron and electron-phonon scattering in ultrathin films. The hot-electron injection efficiency from monocrystalline gold into TiO2, approaching 9% is measured, close to the theoretical limit. These experimental and modelling results reveal the important role of crystallinity and interfaces on the microscopic electronic processes important in numerous applications.

==> sections/OldVersions/ServiceFile.tex <==
Introduction:

The dielectric function of a material $\epsilon = \epsilon_1 + i\epsilon_2$, which describes its optical properties, is influenced by the band structure, which is seen in Fig. \ref{fig:1}d, as it relates to the allowed electronic transitions and the density of states in the material. $\epsilon_$ is strongly influenced by both intraband and interband transitions, where intraband transitions arise from the excitation of electrons within the broad s and p-bands, while interband transitions occur between the d-band and higher lying s- and p-bands, leading to its distinctive optical properties in the visible and near-infrared spectral range \cite{https://doi.org/10.1002/adom.201300457,PhysRevB.86.235147}. As can be seen in Fig. \ref{fig:1}c, for the calculation details see SI-A, $\epsilon_2$ of Au is well described by Drude response by intraband transitions up to approximately photon energy of 1.8 eV and above is described with the additional interband terms which are the transitions from d-band to p-band transition at X symmetry point at 1.8 eV, from d-band to p-band at 2.4 eV, and from p-band to s-band at 3.5eV.  

In order to design and optimize the performance of hot carrier devices, a detailed microscopic understanding of their properties and thermalization dynamics is essential. The prompt energy distribution of the photoexcited hot carriers is closely related to the allowed electronic transitions and the density of states in the solid. Thus, it depends on the energy of the incident photon and the material band structure and is closely connected to the dielectric function of the metal, $\epsilon = \epsilon_1 + i\epsilon_2$, which describes its optical properties.  For example, for Gold (Au), both intraband and interband transitions are possible, leading to its distinctive optical properties in the visible and near-infrared spectral range \cite{https://doi.org/10.1002/adom.201300457,PhysRevB.86.235147}.  Intraband transitions arise from the excitation of electrons within the broad s and p-bands and dominate for photon energies below $h\nu <1.8 eV$. In this range, $\epsilon_2$ of Au is well described by a Drude response (Fig. \ref{fig:1}c). Interband transitions, instead, occur at specific points in the band-structure, i.e. around specific photon energies. For Au, these occur at X point ($\approx 1.8 eV$, d-band to p-band transition) and at L-point ($\approx 2.4 eV$, d-band to p-band and $\approx 3.5eV$, p-band to s-band).  


OPTION 2: 
Monocrystalline (MC) metals have recently emerged as a major research focus in the field of plasmonics. Indeed, their unique optical properties make them highly attractive for a wide range of applications, from sensing and imaging to information processing and energy harvesting  \cite{cite-key,doi:10.1021/acs.chemmater.1c03908,Anatoly2022}. In particular, thanks to the highly ordered crystal structure and lack of grain boundaries (Fig. \ref{fig:1}a) they allow for long-range coherence and reduced optical losses. These are typically exploited to achieve higher resonance quality factors, longer surface plasmon polariton propagation lengths, and superior electric field confinements compared to polycrystalline (PC) metals \cite{doi:10.1063/1.2987458,Lebsir2022} . Concurrently, advancements in the synthesis of monocrystalline metallic platelets towards larger lateral sizes, higher aspect ratios, and pristine (ligand-free) surfaces, have broadened the availability of these substrates.  \cite{doi:10.1021/acs.chemmater.1c03908,KalteneckerKraussCassesGeislerHechtMortensenJepsenStenger+2020+509+522} WE NEED MORE REFRENCES. Interestingly, MC metals could uniquely benefit plasmonic charge transfer devices, such as photodetectors and photoelectrodes. In fact, these devices rely on the injection of  photoexcited energetic (hot) electrons or holes, with excess energy above their thermal equilibrium state, from the metal into an into an adjacent semiconductor or adsorbed molecule. Thus, reduced scattering losses could favor ballistic hot carrier collection and improve the performance of these devices. 


Moreover, the precise control over the plasmonic properties of monocrystalline metals through crystallographic orientation and lattice spacing enables tailored manipulation of plasmonic behavior, which can lead to advanced plasmonic functionalities and device performance. The advancements in fabrication techniques, such as synthesized colloidal monocrystalline Au platelets \cite{doi:10.1021/acs.chemmater.1c03908,KalteneckerKraussCassesGeislerHechtMortensenJepsenStenger+2020+509+522} with atomically smooth surfaces through chemical processes and nanoimprint lithography, have also made it possible to create complex and well-defined plasmonic structures in monocrystalline metals, opening up new possibilities for designing and engineering plasmonic devices with superior performance \cite{Barcelo2016}.  

Hot carriers in plasmonic (metallic) nanostructures, i.e. energetic electrons or holes with excess energy above their thermal equilibrium state, have attracted growing attention due to their unique properties and potential for optoelectronic and energy applications \cite{reference2,reference3,Brongersma2015}. Indeed, thanks to their high kinetik energies, these carriers play an important role in charge transfer devices. In particular,  they can be injected into an adjacent semiconductor, enabling sub-bandgap photodetection and paving the way to miniaturized, on-chip spectrometers ADD REFS \cite{Tagliabue2020,Tagliabue2020_2}. Concurrently, benefiting from the excellent catalytic properties of plasmonic metals, they can be transferred to the empty levels of adsorbed molecules,  altering the photo(electro)chemical reaction pathway and improving selectivity for desired products ADD REFS \cite{doi:10.1021/acs.jpcc.7b12080,DuChene2018}. 



Monocrystalline (MC) metals have recently emerged as a major research focus in the field of plasmonics thanks to their unique optical properties. In particular, because of the highly ordered crystal structure and lack of grain boundaries (\textbf{Fig. \ref{fig:1}a}) they allow for long-range coherence and reduced optical losses. These have been shown to enable higher resonance quality factors, longer surface plasmon polariton propagation lengths, and superior electric field confinements compared to polycrystalline (PC) metals \cite{doi:10.1063/1.2987458,Lebsir2022}. Concurrently, advancements in the synthesis of MC metallic microflakes, in particular Gold (Au) ones, towards larger lateral sizes and higher aspect ratios, has enabled the study and exploitation of these outstanding physical properties in ultra-thin (sub-15nm) films, which are of difficult realization with PC metals.  \cite{doi:10.1021/acs.chemmater.1c03908,KalteneckerKraussCassesGeislerHechtMortensenJepsenStenger+2020+509+522} While MC metals are overall attractive for a wide range of plasmonic applications, from sensing and imaging to information processing and energy harvesting  \cite{cite-key,doi:10.1021/acs.chemmater.1c03908,Anatoly2022} they could uniquely benefit plasmonic charge transfer devices, such as photodetectors and photoelectrodes ��reference2,reference3,Brongersma2015. These systems indeed rely on the injection of photoexcited highly energetic (hot) electrons or holes from the metal into an into an adjacent semiconductor, enabling sub-bandgap photodetection, or adsorbed molecule, triggering photochemical reactions with altered pathways and selectivity ��doi:10.1021/acs.jpcc.7b12080,DuChene2018. Reduced scattering losses could thus favor ballistic hot carrier collection, significantly improving device performance. Additionally, well-defined crystal facets in MC metals would help clarify the interplay of catalytic properties and hot carrier injection in plasmonic photoelectrodes. Yet, limited works have explored the use of MC metals in hot carrier devices (TO BE DISCUSSED).   

\textbf{Proposed Logical Sequence for Introduction} (I indicated which questions we want to address in each paragraph in order to highlight best the importance of our results):
\begin{itemize}
    \item \textit{Why monocrystalline metals are exciting?} Recently, monocrystalline metals have emerged as an attractive platform for fundamental studies and device development, thanks to [mention advantages of monocrystalline metals and cite works that have USED these metals, in particular gold]
    \item \textit{How can monocrystalline metals benefit plasmonic hot carrier devices?}Hot carrier devices are attracting growing interest across optoelectronic and energy applications. In particular, coupled with nanophotonic and plasmonic engineering that enables coupling of light to dimensions comparable to their mean free paths. 
    \item \textit{What is known about hot carriers in metals ?} Understanding how hot carrier dynamics is influenced by the material properties it is critical for device design and optimization. 
    \begin{itemize}
        \item RECAP the known hot carrier dynamics (interband/intraband generation - non thermal distribution; thermalization - e-e and e-ph scattering).  Mention how this relates to collection for efficient applications. "Therefore, the hot carrier dynamics is profoundly affected by the physical properties of the material". 
        \item RECAP Literature review on ultra-fast studies on plasmonic metals (say what has been measured so we can clarify how how work fills a knowledge gap).
    \end{itemize}
    \item \textit{What remains to be understood in hot carrier dynamics ?} Overall, despite the attractiveness of monocrystalline metals, few works have addressed specifically these materials. In particular, when considering the ultra-thin regime, there is a lack of data. (elaborate more here) Yet, because of their unique material structure, it is unclear how the dynamics of hot carriers are affected. 
    \item \textit{What do we do in this paper?} In this work, we study.....\textit{See bullet-points below}
    \item \textit{What is the BROAD IMPACT of this paper?} Overall, our results ....
\end{itemize}




==> sections/OldVersions/section01.tex <==
\section{Introduction} \label{sec:Intro}
\checkmark
\textbf{Proposed Logical Sequence for Introduction} (I indicated which questions we want to address in each paragraph in order to highlight best the importance of our results):\checkmark
\begin{itemize}
    \item \textit{Why studying hot carriers in metals?}Hot carrier devices are attracting growing interest across optoelectronic and energy applications. In particular, coupled with nanophotonic and plasmonic engineering that enables coupling of light to dimensions comparable to their mean free paths. 
    \item \textit{Why considering monocrystalline metals?} Recently, monocrystalline metals have emerged as an attractive platform for fundamental studies and device development, thanks to [mention advantages of monocrystalline metals and cite works that have USED these metals, in particular gold]
    \item \textit{What is known about hot carriers in metals ?} Understanding how hot carrier dynamics is influenced by the material properties it is critical for device design and optimization. 
    \begin{itemize}
        \item RECAP the known hot carrier dynamics (interband/intraband generation - non thermal distribution; thermalization - e-e and e-ph scattering).  Mention how this relates to collection for efficient applications. "Therefore, the hot carrier dynamics is profoundly affected by the physical properties of the material". 
        \item RECAP Literature review on ultra-fast studies on plasmonic metals (say what has been measured so we can clarify how how work fills a knowledge gap).
    \end{itemize}
    \item \textit{What remains to be understood in hot carrier dynamics ?} Overall, despite the attractiveness of monocrystalline metals, few works have addressed specifically these materials. In particular, when considering the ultra-thin regime, there is a lack of data. (elaborate more here) Yet, because of their unique material structure, it is unclear how the dynamics of hot carriers are affected. 
    \item \textit{What do we do in this paper?} In this work, we study.....\textit{See bullet-points below}
    \item \textit{What is the BROAD IMPACT of this paper?} Overall, our results ....
\end{itemize}

Hot carriers, energetic electrons or holes with excess energy above their thermal equilibrium state, in metals have attracted significant attention in recent years due to their unique properties and potential for various  research fields \cite{reference2,reference3,Brongersma2015}. These carriers, while having very high energies, are still bound to the nanostructure they are part of and play an important role in charge transfer devices \cite{Tagliabue2020,Tagliabue2020_2} and chemical reactions, as they can be transferred to nearby structures and trigger photochemical reactions by filling empty levels in acceptor molecules \cite{doi:10.1021/acs.jpcc.7b12080,DuChene2018}. The factors that can affect the energy distribution of hot carriers in a material include the energy of incident photons, and plasmon excitation, material properties such as band structure and scattering mechanisms, carrier-phonon and carrier-carrier interactions\cite{Heilpern2018,Sundararaman2014}. The study of hot carriers in metals has not only advanced our understanding of fundamental physics but has also paved the way for a wide range of technological applications. These applications 
include electronics with high frequency and power 
\cite{doi:10.1063/1.4961874,doi:10.1063/1.1896479}, where the rate at which charges are 
transported is determined by how quickly they relax, as well as photothermal treatments 
\cite{C6RA11130K,HUANG201013} and laser machining using ultrafast laser sources 
\cite{reference1,doi:10.1063/1.370197}, where the rate at which electrons become connected to vibrational states plays a significant role in the amount of heat produced locally.  


The dielectric function of a material $\epsilon = \epsilon_1 + i\epsilon_2$, which describes its optical properties, is influenced by the band structure, which is seen in Fig. \ref{fig:1}d, as it relates to the allowed electronic transitions and the density of states in the material. $\epsilon_$ is strongly influenced by both intraband and interband transitions, where intraband transitions arise from the excitation of electrons within the broad s and p-bands, while interband transitions occur between the d-band and higher lying s- and p-bands, leading to its distinctive optical properties in the visible and near-infrared spectral range \cite{https://doi.org/10.1002/adom.201300457,PhysRevB.86.235147}. As can be seen in Fig. \ref{fig:1}c, for the calculation details see SI-A, $\epsilon_2$ of Au is well described by Drude response by intraband transitions up to approximately photon energy of 1.8 eV and above is described with the additional interband terms which are the transitions from d-band to p-band transition at X symmetry point at 1.8 eV, from d-band to p-band at 2.4 eV, and from p-band to s-band at 3.5eV.  

The way in which the distribution of hot carriers, also called nonthermal carriers, changes, electron temperature T$_e$, and lattice temperature T$_l$, over time follows predictable dynamics by a three-temperature model (3TM). 3TM, which accounts for the energy density stored in nonthermal carriers $N_e$, $T_e$ and $T_l$, is the framework in which the link between non-equilibrium energy transfer rates and the measured optical response is most frequently interpreted in metals\cite{PhysRevB.50.15337,Zavelani-Rossi2015}. Briefly, photon absorption instantaneously excites the carriers in the pulse length of the laser and increases $N_e$ as can be seen in Fig. \ref{fig:1}e. Then this energy is quickly exchanged through scattering with other carriers,
which takes a thermalization lifetime $\tau_{th}$ of a few hundred femtoseconds. Once the 
carriers have reached an internal equilibrium, they are called thermalized carriers, and they transfer their thermal energy to the phonons 
(vibrational units of a crystal lattice), and the distribution of carriers equilibrates at 
$\tau_{e-ph}$ that takes a few picoseconds \cite{Jiang2013,Biagioni2012,Méjard2016}. Progressively, the thermalized phonons of the lattice interact with the phonons of the surrounding media, and the thermal equilibrium is reached. The dynamics of hot carriers can be investigated using a technique called pump-probe measurement. This involves using a high-intensity laser pulse to excite a large number of electrons in a plasmonic material and measuring the structure's optical response over time using a delayed probe pulse. This method has been used in various studies to examine processes such as e-e and e-ph scattering, and electronic transport \cite{https://doi.org/10.1002/lpor.202000346,BykovRothSartorelloSalmónGamboaZayats+2021+2929+2938,C3EE42731E,PhysRevB.50.15337,PhysRevB.61.16956}. Fig. \ref{fig:1}f shows the typical probe energy dependence of $\Delta R/R$ at different time frames. In this simulation, we used the theory described in SI-A and computed the case for 1.7 eV pump causes $\Delta T_e$=1000K by ignoring the L point p-band to s-band transitions at 3.5 eV since it is out of the focus of this study. 
\begin{figure} [h!]
    \centering
    \includegraphics[keepaspectratio,height=21cm, width=12.5cm]
    {images/Fig1_GT_V0.eps}
    \caption{\justifying{a)The degenerate back surface pumping and front surface probing configuration used in $\Delta R/R$ measurements at 1.7 eV by 8 fs pulses. b) Schematic illustration of the possible scattering mechanisms in monocrystalline Au and polycrystalline Au. c) the measured and computed imaginary part of the dielectric function of Au. The data, which are dots, is taken from Johnson and Christy \cite{PhysRevB.6.4370} and the computation is done by considering the Drude term and the interband transitions at X and L points of the Brillouin zone(See SI-A.). d) Electronic band structure of Au reprinted from ??. e) Example of calculated transient energy density stored in non-thermal electrons,$N_e$, $T_e$, and $T_l$ by 3-TM at 1.7 eV and F=6 ($J/m^2$) for 10 nm Au. The inset describes the typical time dynamics of the energy stored in the system after the photon absorption. f) Computed probe energy dependence of $\Delta R/R$ for $\hbar \omega_{pump}=1.7eV $ and $\Delta T_e$=1000K. }}
    \label{fig:1}
\end{figure}

Furthermore, monocrystalline metals have emerged as a significant research focus in the field of plasmonics due to their unique and enhanced plasmonic properties. The highly ordered crystal structure and lack of grain boundaries of monocrystalline metals, which can be seen in Fig. \ref{fig:1}b, allows for long-range coherence and reduced scattering losses, resulting in improved plasmonic performance compared to polycrystalline metals \cite{doi:10.1063/1.2987458,Lebsir2022}. Therefore, monocrystalline metals exhibit higher quality factors, longer propagation lengths, and superior field confinement, making them attractive for various plasmonic applications such as sensing, imaging, energy harvesting, and information processing \cite{cite-key,doi:10.1021/acs.chemmater.1c03908,Anatoly2022}. Moreover, the precise control over the plasmonic properties of monocrystalline metals through crystallographic orientation and lattice spacing enables tailored manipulation of plasmonic behavior, which can lead to advanced plasmonic functionalities and device performance. The advancements in fabrication techniques, such as synthesized colloidal monocrystalline Au platelets \cite{doi:10.1021/acs.chemmater.1c03908,KalteneckerKraussCassesGeislerHechtMortensenJepsenStenger+2020+509+522} with atomically smooth surfaces through chemical processes and nanoimprint lithography, have also made it possible to create complex and well-defined plasmonic structures in monocrystalline metals, opening up new possibilities for designing and engineering plasmonic devices with superior performance \cite{Barcelo2016}. Overall, the use of monocrystalline metals in plasmonics has become increasingly important due to their enhanced plasmonic properties, precise control over plasmonic behavior, and potential for advanced plasmonic applications. Overall, despite the attractiveness of monocrystalline metals, few works have addressed specifically these materials. While the properties of the plasmonic materials, including their topography\cite{LARENA2002339}, thickness \cite{PhysRevLett.92.026808}, and crystallinity\cite{PhysRevB.86.235147}, have been studied and found to have a significant impact on the optical properties, the hot carrier dynamics are still not well elucidated. In particular, when considering the ultra-thin regime, it is unclear how the dynamics of hot carriers are affected.

\textbf{Main results}:\checkmark
\begin{itemize}
    \item Observation of the role of thermalized carriers on the transient signal at IR pump/probe. This shows that the X-point transition is important and that, at high electron temperatures this term must be accounted for. 
    \item Longer e-e thermalization time for the MC sample compared to PC. This shows the role of grain boundaries in the e-e thermalization. 
    \item Shorter e-ph thermalization for MC compared to PC. Due to higher e-ph coupling comapred to PC (Do we have an explanation?) 
    \item Signature of hot-electron transfer on the MC TA signal at short time-scales (non-thermalized carriers gets removed, larger relative contribution of thermalized carrier on the signal)
    \item Estimate of injection probability from e-ph coupling in MC/TiO2 sample. Approx 10\% efficiency is an interesting result considering the ultra-low roughness of the Au surface. 
    \item Trend of e-ph coupling time on thinkness and fluence. 
\end{itemize}

Here we investigate the effect of crystallinity and thickness of Au on hot carrier generation, relaxation, and transfer dynamics down to 10 nm thickness by degenerate near-IR, 1.7 eV, $\Delta R/R$ measurements with 8 fs laser pulses. We show the delayed rise of $\Delta R/R$  due to a decrease in $\gamma_{ee}$ in the case of monocrystalline Au MF because of a lack of grain boundaries compared to polycrystalline Au. Our studies indicate that as the perturbation increases with the increase in $T_e$, the effect of the X point interband transitions in Au must be accounted and it increases the contribution of long-lived thermalized electrons and causes a delayed rise in $\Delta R/R$ even at the pump energy of 1.7 eV. We also show the  delayed rise of $\Delta R/R$ in the presence of hot electron transfer from Au to TiO$_2$ due to a decrease in the nonthermal electron contribution to the signal. Even in the case of hot electron transfer, much longer e-ph relaxation is observed on a thermally low conductive substrate. We also showed that the perturbation regimes have an impact on the thicknesses dependence of $\tau_{e-ph}$. We find the hot electron injection efficiency $\approx$ 9$\%$ close to the theoretical limit, although the Au surface is atomically flat. This finding is highly promising for hot carrier transfer devices with monocrystalline metals, allowing efficient surface plasmon resonances thanks to their atomically flat surfaces. A semiclassical approach based on transient dielectric function computation by considering both interband transitions and Drude formalism coupled with 3TM is exploited to explain the observed dynamics quantitatively.

==> sections/OldVersions/section02.tex <==
\section{Methods} \label{sec:Methods}

\textbf{Comment}: I would put part of this info as the first paragraph of the Results section. In particular, we need to provide the most important info to the reader upfront (i.e. technique, pulse length and wavelength, samples etc.). Such a dedicated Method section will go at the end of the manuscript instead, as typically done in journals like Nature Comm the method section. So the reader would not see this immediately info when reading the manuscript. 



==> sections/OldVersions/section03.tex <==
\section{Results and Discussion} \label{sec:Results }

\textbf{Sequence and Critical points to be discussed} (you already have most of them, I am just trying to check here what is missing as well as the overall flow of the different paragraphs):
\begin{itemize}
\item \textit{Missing in current version} Describe briefly the studied samples and experimental conditions (Fig 1) \checkmark
\begin{itemize}
    \item In our study we compare 10nm polycrystalline gold films deposited by evaporation on a borosilicate substrate with monocrystalline flakes synthetized.... 
    \item We use transient absorption spectroscopy (reflection configuration) to study the hot carrier dynamics in these two systems. Uniquely, we use a 8fs pump pulse with central wavelength in the IR (see Supplemetary XX - spectrum). Also, we use a weaker probe with the same spectrum. 
\end{itemize}
\item \textit{Missing in current version} Discuss the role of intra- and inter band transitions and how this experimental configuration makes us very sensitive to the non-thermal carrier dynamics (Use the new Fig 1 to explain the expected signal and what is thermal and what is non-thermal. Currently you only CITE literature to say this is the case but we really need the reader to understand the point, so we have to explain it). \checkmark
\item e-e thermalization (Fig 2):\checkmark
\begin{itemize}
    \item Present the results on the e-e thermalization highlighting the difference between MC and PC as a function of Fluence (Fig 2a).
    \item \textit{Partially missing in current version = extend with more info} Discuss the model, using the polycrystalline film as a function of fluence as the calibration case. 
    \begin{itemize}
        \item Explain the concept behind the model (relate the change in epsilon to the population of thermal and non-thermal carriers)
        \item Discuss band structure and epsilon. Introduce the X point and the L point. 
        \item Report the critical equations of the model from SI (i.e. A8 - Im(DeltaEpsilon), A9 - JDOS) 
        \item         Explain the effect of Te(t) onto the smearing of the X-point JDOS. 
        \item Show the relative contribution of N(t) and Te(t) as a function of Fluence onto the change in epsilon T(NT) and link it to the observed transient signals. (refer to theory plots such as Ne(t), Te(t) and epsilon Thermal/NonThermal (t) (see new Fig 2).
    \end{itemize}
    \item Compare PC and MC with the model and discuss the origin of the difference
    \item Present the result for MC on SiO2 and TiO2 and explain the difference.
\end{itemize}
\item e-ph thermalization and injection probability (Fig 3 and 4)\checkmark
\begin{itemize}
    \item Compare PC and MC and discuss the increase in G (Fig 3)
    \item Compare MC on SiO2 and TiO2 and discuss the role of Pinj (Here I would move most of the equations in SI, making a new SI section about Pinj. I would keep only Eqn (5) of the current version) (Fig 3)
    \item Comment on the achieved value of Pinj
    \item Discuss the role of thickness and fluence (Fig 4)
\end{itemize}
\end{itemize}


\textbf{Experiments}. 
The high aspect-ratio ultrathin monocrystalline Au MFs are fabricated by the procedure described by Kiani et al \cite{doi:10.1021/acs.chemmater.1c03908}. MF has atomically smooth and well-defined $\{111\}$ crystallographic surface and face-centered cubic crystal structure.The used substrate is 180$\mu$m thick 
borosilicate glass. To study the hot electron transfer, the chemically synthesized flakes are 
transferred to the 40nm thick TiO$_2$ on borosilicate glass by PMMA transferring method 
\cite{https://doi.org/10.1002/smtd.201900049}. The studied range of the flake thickness is 10-25nm. To compare the effect of crystallinity on hot-carrier dynamics, 10 nm thick Au thin-film samples are fabricated on the same type of substrate by sputtering. Note that AFM analysis verifies that there is no discontinuity on the 10 nm thick Au thin film. The transient optical measurements were conducted using an 8 fs-long laser (Laser Quantum Venteon) in the degenerate back surface pumping and front surface probing configuration, as can be seen in Fig.\ref{fig:1}a. The center energy of the laser is 1.7 eV. For additional experimental details, please see the Methods section.





\begin{figure} [h!]
    \centering
   \hspace*{-3cm}   
   \includegraphics[keepaspectratio,height=27cm, width=20cm]
   {images/Fig2_GT_V3.eps}
    \caption{\justifying{a) The instantaneous change in  the nonthermal electron distribution change, $\Delta \rho_{nonthermal}$, (orange curves) of the 1.7 eV pump laser and corresponding thermalized electron distribution change, $\Delta \rho_{thermal}$,(blue curves) vs electron energy from  $E_F$ at $\Delta T_e$=50K, 500K and 1000K. b) Measured rise of $\Delta R/R$ of 10 nm thick monocrystalline Au MF(purple curves) and polycrystalline Au (green curves) on SiO$_2$ at F=3.6 ($J/m^2$) (dashed curves) and F=5.7 ($J/m^2$) (solid curves). The inset shows the low perturbation $\Delta R/R$ measurement at F=0.3 $(J/m^2)$. c) Transient change in the imaginary part of the dielectric function of Au caused by nonthermalized electrons $\Delta \epsilon_{NT}$ (blue curves) and thermalized electrons $\Delta \epsilon_{T}$ (orange curves)at F=0.25,2.5 and 5 $J/m^2$ at $\hbar\omega=1.7 eV$. d) Computed (cyan curves) and measured (green curves) $\Delta R/R$ of 10 nm thick polycrystalline Au on SiO$_2$  at F=3.6 ($J/m^2$) (dashed curves) and F=5.7 ($J/m^2$) (solid curves). Inset shows the JDOS at the X-symmetry point at several electron temperatures. e) Computed (cyan curves) and measured (purple curves) $\Delta R/R$ of 10 nm thick monocrystalline Au MF on SiO$_2$  at F=3.6 ($J/m^2$) (dashed curves) and F=5.7 ($J/m^2$) (solid curves). Inset shows the calculated JDOS at the X-symmetry point for monocrystalline (purple curves) and polycrystalline (green curves) Au. f) Measured rise of $\Delta R/R$ of 10 nm thick monocrystalline Au MF on SiO$_2$ (purple curves) and on TiO$_2$ (red curves)  at F=3.6 ($J/m^2$) (dashed curves) and F=5.7 ($J/m^2$) (solid curves). Inset shows the low perturbation $\Delta R/R$ measurement at F=0.3 $(J/m^2)$.}}
    \label{fig2}
\end{figure}
\

 
  

\textbf{e-e scattering and electron thermalization}. Applying a short-duration pump pulse to a material can alter the electron distribution without changing the lattice temperature. If the energy of the pump photons is much lower than the energy needed for interband transitions, then only free-carrier absorption affects the electron distribution, leaving the d-band electrons unaffected. This can result in a broad non-Fermi distribution of nonthermal electrons above the Fermi level, extending up to the energy of the pump photons. Because the density of states in Au remains nearly constant near the Fermi energy \cite{PhysRevB.4.3321}, the change in the electron distribution due to instantaneous excitation can be mathematically expressed as \cite{PhysRevB.50.15337}
  \begin{equation} \label{rhoNT}
      \Delta\rho_{NT}(\varepsilon)=Cf_0(\varepsilon-\hbar\omega_{pump})[1-f_0(\varepsilon)]-f_0(\varepsilon)[1-f_0(\varepsilon+\hbar\omega_{pump})].
  \end{equation}
where $f_0$ is the Fermi distribution at 293K, $\varepsilon$ is the electron energy, C is the parameter depends on the pump intensity, and $\hbar\omerga_{pump}$ is the pump photon energy which is 1.7 eV in our experiments. By e-e scatterings, the energy stored in the nonthermal electrons is redistributed and creates Fermi distribution of $ \Delta \rho_T(\varepsilon,t) \propto f_0(\varepsilon,T_e(t))-f_0(\varepsilon,T_0)$ where $T_e>T_0$ \cite{Zavelani-Rossi2015}. Fig.\ref{fig2}a shows the $\Delta\rho_{NT}$ and $\Delta\rho_{T}$ for different $\Delta T_e$. As can be seen that after the relaxation of the nonthermal electrons, the change in the thermalized electron distribution is localized around $E_F$ and smearing with the temperature.  It is known that the rise time of transient signal highly depends on the pump and probe wavelengths. The thermalized electrons in noble metals contribute less at probe wavelengths that are farther away from the resonant d band to Fermi-surface transitions, i.e. in the case of non-resonant probing, and nonthermal signals become relatively more important \cite{PhysRevLett.118.087401}. While in non-resonant near-IR probing the rise in the transient signal is mostly dominated by non-thermal electrons as an instantaneous rise in the transient signal, probing the d-band to Fermi surface transitions allows probing the internal thermalization dynamics, i.e. it allows to probe long-lived thermalized carriers localized at Fermi level $E_F$ \cite{PhysRevB.61.16956}. Therefore, in near-IR probing, the rise in $\Delta R/R$ is mostly dominated by non-thermal electrons as an almost instantaneous rise happens in 200 fs in our experiments. It is significantly faster than the expected electron thermalization time, $\tau_{th}$, which is around 500fs for Au and can be measured by resonant interband probing \cite{PhysRevB.61.16956,PhysRevB.50.15337,PhysRevB.46.13592}.

As can be seen in Fig. \ref{fig2}b, as the laser fluence increases, the rise of $\Delta R/R$ is delayed. We attribute this to the increase in the relative contribution of the thermalized electrons near $E_F$ compared to nonthermal electrons to $\Delta R/R$. An increase in the laser fluence results in the build-up in the electron temperature.  Although the general perception is that interband transitions start after 2.5 eV, it is known to start after 1.85 eV, albeit with less efficiency \cite{PhysRevB.12.4570}. While this region covers a tiny portion of our laser spectrum, the interband transitions become more important and need to be taken into account at higher $T_e$ as can be seen in JDOS calculation at X point in the inset of Fig.\ref{fig2}d. It leads to a broadening of the Fermi distribution and the increase in the long-lived thermalized electron occupancy near $E_F$. To investigate the effect of transient interband transitions on permittivity, the temporal variation in the permittivity of Au can be defined as 
\begin{equation}\label{temp_epsilon}
\Delta\epsilon(\hbar\omega,t)=\Delta\epsilon_{NT}(\hbar\omega,t)+\Delta\epsilon_{T}(\hbar\omega,t)+\Delta\epsilon_{Drude}(\hbar\omega,t)
\end{equation}
where the sum of thermalized, nonthermal and Drude terms. The temporal dynamics of each component are obtained by introducing the 3TM parameters of $N_e$, $T_e$, and $T_l$ into JDOS calculation under constant matrix element approximation with parabolic band approximation for $\epsilon_{NT}$ and $\epsilon_T$ and into Drude-Sommerfeld model for $\epsilon_{Drude}$(see \ref{sec:appendix_SI1}) \cite{PhysRevB.12.4570,Zavelani-Rossi2015}. The higher scaling up in the amplitude of $\Delta\epsilon_{2T}(t)$ compared to $\Delta\epsilon_{2NT}(t)$ can be seen in our calculations in Fig. \ref{fig2}c as the laser fluence increases, which is the driven source of the increase in $\tau_{rise}$ with the laser fluence. From the ab initio calculations done by Brown et al. and/or by Del Fatti et al., it is shown that $\tau_{th}$ decreases with the laser fluence because of significant smearing of the electron distribution around the Fermi energy and the concurrent increase of the e-e scattering efficiency due to the weakening of the effects of the Pauli exclusion.\cite{PhysRevLett.118.087401, PhysRevB.61.16956}. While decreasing the $\tau_{th}$ with the fluence, an increase in the ratio between the amplitudes of the thermalized and nonthermalized electrons contribution leads to an increase in $\tau_{rise}$, and accurately estimated with our model for both polycrystalline and monocrystalline Au as be seen in Fig.\ref{fig2} d and e, respectively.(see \ref{sec:appendix_SI1}).

 As can be seen in Fig. \ref{fig2}b, as the laser fluence becomes perturbative, the rise of $\Delta R/R$ in polycrystalline Au thin film is faster than in monocrystalline Au MF. The low perturbation measurements, in which the rise in $\Delta R/R$ is mostly dominated by nonthermal electron contribution because of a tiny change in the electron temperature, $T_e$, can be seen in Fig \ref{fig2}b as an inset, show that the nonthermal electron contribution to the rise is the same for both cases. We attribute this delayed rise of $\Delta R/R$ in monocrystalline Au at high perturbation to two aspects, which are the difference in the $\gamma_{ee}$ between monocrystalline and polycrystalline Au and optical transitions from occupied states in d-bands to p-bands quasi-free states at X-symmetry point of the Brillouin zone. First, the study conducted by Henriquez et al. shows that the grain nature of the polycrystalline films increases the scattering rate with the mechanism of electron-grain boundary scattering \cite{doi:10.1063/1.4791600}. As the grain sizes decrease, the electron-grain boundary scattering also increases. Olmon et al. also shows that the increase in the Drude damping parameter, which is electron scattering rate, $\gamma_{ee}$, also increases in the case of polycrystalline compared to the monocrystalline Au \cite{PhysRevB.86.235147}. Because the monocrystalline Au MFs lack grain boundaries, they do not have any contribution from grain boundary scattering. Since $\tau_{th} \propto \gamma_{ee}^{-1}$, $\tau_{th}$ is longer in the case of monocrystalline Au MF than polycrystalline Au, and the thermalized electron contribution to $\Delta R/R$ is delayed. Fig. \ref{fig2} d and e show the computed $\Delta R/R$ for poly and monocrystalline Au at different fluences based on the model described in SI, respectively. Latter, the measured optical dielectric function of polycrystalline Au by Johnson and Christy, and monocrystalline Au by Olmon et.al. show that the optical transitions at the X symmetry point are slightly stronger in monocrystalline Au compared to polycrystalline Au, which can also be seen in the inset of Fig. \ref{fig2}e by our JDOS calculation at 1000K electron temperature based two measurements \cite{PhysRevB.86.235147,PhysRevB.6.4370}. Since the higher number of interband transitions in monocrystalline Au means a higher number of excited electrons near E$_F$, which are long-lived, it turns out the delayed rise in $\Delta R/R$ in monocrystalline Au MF compared to polycrystalline Au.   

We continue our discussion with the differences between $\tau_{rise}$ in the cases of 10 nm thick Au MF on SiO$_2$, and on TiO$_2$ and discuss the relative contributions of thermalized and nonthermalized electron contributions to the rise of $\Delta R/R$ in these cases. When an n-type semiconductor material such as TiO$_2$ and a metal form a junction, electrons flow from the semiconductor to the metal to equalize their $E_F$. This causes the energy levels of the conduction and valence bands in the semiconductor to bend upwards as one moves from the interior of the semiconductor to the semiconductor-metal contact, as can be seen in Fig.\ref{fig2}f. This results in the formation of a Schottky barrier at the interface, which is the energy difference between the original E$_F$ of the metal and the semiconductor. An electron can only transfer from the metal to the semiconductor if it has enough energy to either overcome or tunnel through the Schottky barrier, which typically has a value ranging from 0.9 to 1.2 eV \cite{Mubeen2011,Ng2016,Ratchford2017}. As can be seen in Fig. \ref{fig2}e, at the same fluence level, the rise of $\Delta R/R$ of Au MF on SiO$_2$ is faster than on TiO$_2$. We attribute this behavior to two different effects: the transfer of highly energetic nonthermal electrons from Au to TiO$_2$ in the first 100fs before participating in the thermalization, and the longer thermalization time since the presence of less energetic carriers, i.e., the rest of the electrons, which do not participate to the transfer, will closer to $E_F$, so they will have a longer lifetime. Thanks to the transfer of the most energetic electrons, the instantaneous rise of $\Delta R/R$ is suppressed. In the low perturbation measurements, in which the
instantaneous response is supposed to dominate the rise in $\Delta R/R$ because of a small $\Delta T_e$, which can be seen as an inset in Fig. \ref{fig2}f, the instantaneous response of nonthermalized electrons has less influence in the case of Au MF on TiO$_2$ than on SiO$_2$ due to the portion of the most energetic electrons being transferred. For the latter, since the rest of the electrons are less energetic, and it is known that $\gamma_{ee}$ is quadratically proportional to the excited electron energy \cite{Zavelani-Rossi2015}, these electrons will be long-lived compared to the case of absence of transfer, as in the case of Au on SiO$_2$. One can also conclude that the most energetic electrons will be transferred, and the rest of the electron gas will heat up less than in the absence of transfer.



\begin{figure} [h!]
    \centering
    \includegraphics[width = 1 \textwidth]{images/Fig3-01.eps}
    \caption{\justifying{a) Measured $\Delta R/R$ of 10 nm thick monocrystalline Au MF (purple curves) and polycrystalline Au (green curves) on SiO$_2$ at F=3.6 ($J/m^2$) (dashed curves) and F=5.7 ($J/m^2$) (solid curves). b) Measured $\Delta R/R$ of 10 nm thick monocrystalline Au MF on SiO$_2$ (purple curves) and on TiO$_2$ (red curves)at F=3.6 ($J/m^2$) (dashed curves) and F=5.7 ($J/m^2$) (solid curves). c) Measured $\tau_{e-ph}$ of 10 nm thick monocrystalline Au MF on SiO$_2$(purple diamonds), on TiO$_2$ (red squares), and polycrystalline Au on SiO$_2$ (green dots) as a function of laser fluence. The dotted curves are computed by Eq\ref{taueph_liter}. for G=1.6x10$^{16} (Wm^{-3}K^{-1})$ (red), G=2x10$^{16} (Wm^{-3}K^{-1})$ (green), G=2.2x10$^{16} (Wm^{-3}K^{-1})$ (purple). d) Measured $\tau_{e-ph}$ of 10 nm thick monocrystalline Au MF on TiO$_2$. The dashed lines are computed Eq \ref{taueph_liter}. for corresponding $P_i$ values in legend.}}
    \label{fig3}
\end{figure}

\textbf{e-ph relaxation.} We continue our discussion with the effect of crystallinity, hot electron transfer, the thermal properties of the substrate, and the thickness of Au on e-ph relaxation. As can be seen in Fig. \ref{fig3}a, e-ph relaxation slows down with the increase in pump fluence, which is a well-known phenomenon as the e-ph relaxation depends on the thermalized electron temperature and as the temperature increases, or the incident pump power increases, relaxation gets longer \cite{Tagliabue2020,PhysRevB.51.11433,Staechelin2021}. Moreover, as can be seen in Fig. \ref{fig3} at the same laser fluence, the e-ph relaxation is slightly faster in monocrystalline Au MF compared to polycrystalline Au thin-film. We attribute the change in $\tau_{e-ph}$ between Au MF and Au thin film to the change in the e-ph coupling constant, G. Based on the simulation results, we determine G$_{MF}$= 2.2x10$^{16} [Wm^{-3}K^{-1}]$ and G$_{thinfilm}$= 2x10$^{16} [Wm^{-3}K^{-1}]$ as an effect of crystallinity on e-ph relaxation. The change in G is not only specific for the case of different crystalline structures but also, there are many different G values reported in the literature in the case of polycrystalline thin films regarding the fabrication methods. Hohlfeld et al. provide a comprehensive table of G values present in the literature \cite{HOHLFELD2000237}. Note that a linear relation between the amplitude of $\Delta R/R$ and incident pump power is observed.

As we discussed above, hot electron transfer happens before electron thermalization. Since the most energetic electrons will be transferred,i.e., since the higher fraction of the initial absorbed energy will be transferred, the rest of the electron gas will heat up less than in the case of the absence of charge transfer. So, one could expect to decrease in $\tau_{e-ph}$ in the case of Au on TiO$_2$. However, as can be seen in Fig. \ref{fig3}b, the situation is reversed as we discussed above. The e-ph relaxation is slower even in the presence of hot electron transfer. We attribute the change in the e-ph relaxations between Au MF on SiO$_2$ and TiO$_2$ to the change in G because of the change in the transfer of thermalized energy stored in the electron directly to the thin film TiO$_2$. There have been numerous studies on how the environment affects $\tau_{e-ph}$ in Au NPs and Au thin film \cite{doi:10.1063/1.125460,https://doi.org/10.1002/adma.200390088,Polavarapu_2009,square_2,HOPKINS20076289}. These findings revealed that $\tau_{e-ph}$ tends to be shorter in environments with higher thermal conductivities. Such as Pamela et al. show that the substrate itself has a significant impact on this behaviour \cite{square_2}. In the experiment, they analyze the Au on Si and on SiO$_2$ and show that the measured G is lower in the case of Au on SiO$_2$ because of the higher thermal conductivity of SiO$_2$. However, others suggest that there is no relation between the substrate and G \cite{PhysRevLett.90.177401}. Even though the thermal conductivity of bulk SiO$_2$, 2$[Wm^{-1}K^{-1}]$ \cite{LIMA201266}, is lower than bulk TiO$_2$ at room temperature, the thermal conductivity of 40 nm thin film TiO$_2$ is 4 times lower than bulk SiO$_2$ \cite{DECOSTER201871}. Moreover, during the mechanical transfer of the flakes to TiO$_2$ coated substrate, there can be a thin layer of water residue between MFs and TiO$_2$ which can also decrease the thermal conductivity. So, these changes in the thermal properties of the underlying medium can induce the observed change in G between these cases and dominate the effect of charge transfer on $\tau_{e-ph}$. Based on the experiments, we determine G$_{SiO_2}$= 2.2x10$^{16} [Wm^{-3}K^{-1}]$ and G$_{TiO_2}$= 1.6x10$^{16} [Wm^{-3}K^{-1}]$ for the Au MF on SiO$_2$ and on TiO$_2$, respectively.





We continue our discussion with the hot electron transfer efficiency of monocrystalline Au MF. Here we use the method of Lehner et al. by doing several modifications (see \ref{sec:appendix_SI2}) \cite{doi:10.1063/1.4870040}. As we discussed above since the most energetic hot electrons inject the fraction of the absorbed energy, $P_i$, into the semiconductor before electron thermalization, the rest of the electron gas will be less heated and the relaxation will be slower. The relation between $\tau_{e-ph}$ and $P_i$ is described in the framework of 3-TM as follows \cite{Staechelin2021,PhysRevB.51.11433}: 
\begin{equation}\label{taueph_liter}
    \tau_{e-ph}\approx \frac{\gamma T_l}{G}+\frac{(1-P_i)U}{2GT_l}
\end{equation}
where $G=G_{TiO_2}$= 1.6x10$^{16} [Wm^{-3}K^{-1}]$, $\gamma$=66$Jm^{-3}K^{-2}$ is the electron heat capacity coefficient for Au. 
By using Eq. \ref{pi_expre}, we calculate P$_i$ for 10 nm thick Au slab with $\phi_b=1 eV$ and $h\nu=1.7 ev$ as 0.12. We also calculate the theoretical limit of P$_i$ as 0.53 by assuming the $\phi_b = 0 eV$ and all excited electrons will reach the interface, i.e. assuming 0 thickness of Au and the momentum towards to interface for all electrons. In Fig. \ref{fig3}d, which shows the lines computed by \ref{taueph_liter} with the calculated P$_i$ values, the dashed line for P$_i$=0.09$\pm$ 0.03 reasonably matches with the experimentally measured $\tau_{e-ph}$ of 10 nm thick Au MF on TiO$_2$. For detailed plots of P$_r$,P$_i$ and P of Au slab on TiO$_2$ and Au nanoparticle embedded inside TiO$_2$, see SI \ref{sec:appendix_SI2}.
\begin{figure} [b]
    \centering
    \includegraphics[width = 0.5 \textwidth]{images/Fig4-01.eps}
    \caption{\justifying {Measured $\tau_{e-ph}$ values of monocrystalline Au of different thicknesses at high (dots), and low perturbation (diamonds) regimes. Solid curves are the computed T$_e$ by 3-TM at high (upper) and low perturbation (lower) regimes. }}
    \label{fig:4}
\end{figure}
Ratchford et al. showed that the injection efficiency, P$_i$, can go up to 25$\%$ in the case of 10 nm Au nanoparticle(NP) embedded in TiO$_2$ at 1.6 eV incident pump \cite{Ratchford2017} (see SI for our calculations). The reason for an around three-fold increase in injection efficiency from Au slab to Au NP embedded in TiO$_2$ is because of the increase in the surface area of the metal-semiconductor interface and the momentum space for transfer \cite{doi:10.1063/5.0029050}. The possible reasons for good agreement between our calculated injection efficiency and measured injection efficiency, and a slight mismatch between our calculations and their measurement can be the difference in the deposition of TiO$_2$, so $\phi_b$, the effect of crystallinity on the ballistic transport of electrons, or the increase in interface area in the case of rough TiO$_2$ surface and Au MF. It has been previously demonstrated that roughness can relax the momentum conservation rule and increase the hot electron current \cite{Goykhman:12}. Even the Au MF has a smooth surface, the underlying non-annealed TiO$_2$ has a rough surface that can still enhance the momentum space for electron transfer. So, it is highly promising that having a good agreement with the calculations under fully-relaxed momentum conservation assumptions can be a sign of an increase in external quantum efficiencies of the hot carrier transfer devices with the use of monocrystalline Au due to efficient plasmon resonances \cite{Qi_2017,Goykhman2011}. Moreover, Ratchford et al. do not observe the change in G since they use Al$_2$O$_2$ and bulk-wise TiO$_2$ as an environment and they have comparable thermal conductivities 10  [$Wm^{-1}K^{-1}$] \cite{Gao2013,doi:10.1063/1.367500}.



Fig. \ref{fig:4} shows the measured $\tau_{e-ph}$ values for different thicknesses of monocrystalline Au MF at low and high perturbation regimes. As can be seen, at a low perturbation regime, i.e. at F= 0.4 $J/m^2$, $\tau_{e-ph}$ decreases as thickness decreases while T$_e$ remains constant. Similar to the impact on e-e scattering, which we showed our calculations about it in SI, electron spill-out reduces average electron density, which leads to less screening and more interaction between the electrons and the ionic lattice, which is thought to be the cause of the decrease in e-ph by Arbouet et al. \cite{PhysRevLett.90.177401}. While these experiments were done in the low perturbation regime, we observe the reversed behaviour at higher fluences, as the thickness decreases $\tau_{e-ph}$ increases. The reason is that as thickness decreases, $\Delta$T$_e$ significantly increases at high perturbation regimes and this makes the e-ph interaction longer. The non-negligible increase in T$_e$, which can be seen in Fig. \ref{fig:4}, suppresses the electron spill-out effect on $\tau_{e-ph}$.

==> sections/OldVersions/section04.tex <==
\section{Conclusion}
In this work, we interrogated the temporal dynamics of hot carriers of monocrystalline Au MFs on SiO$_2$ and on TiO$_2$ and polycrystalline Au thin film on SiO$_2$ in the thickness range of 10 to 25 nm by degenerate near-IR, 1.7 eV, $\Delta R/R$ with 8-fs laser pulses. We showed a difference in the contributions of the thermalized and nonthermalized electrons to $\Delta R/R$ between mono and poly-crystalline Au and also between the cases of presence and absence of hot carrier transfer at different laser fluence levels. We found that longer electron thermalization in monocrystalline Au due to a decrease in $\gamma_{ee}$, which was caused by the absence of grain boundaries, results in the delayed rise of $\Delta R/R$. We also showed the presence of hot electron transfer from Au to TiO$_2$ suppresses the nonthermal electron contribution to $\Delta R/R$ as a delayed rise. We demonstrated that $\Delta R/R$ in non-resonant probing could also show a delayed increase, similar to what is seen in resonant probing under highly perturbative excitation. Contrary to general perception, in the near IR region, Au interband transitions still have great importance on hot carrier dynamics. So, the semiclassical approach, in which we count not only Drude contributions but also the interband transitions, reflects the observed interesting things.Our studies indicate that as the perturbation increases with the increase in $T_e$, the effect of the X point interband transitions in Au must be accounted and it increases the contribution of long-lived thermalized electrons and causes a delayed rise in $\Delta R/R$ even at the pump energy of 1.7 eV. We also found that even when hot electron transfer occurs, there is much longer e-ph relaxation on a thermally low conductive substrate. We demonstrated that the perturbation regime highly affects the thickness dependence of $\tau_{e-ph}$. We found that hot electron injection efficiency is approximately 9$\%$, which agrees with our estimate under momentum relaxation, even though the Au surface is atomically flat. This result is promising for the use of monocrystalline metals in hot carrier transfer devices, as it allows for efficient surface plasmon resonances. We believe these new findings can contribute to understanding the non-equilibrium dynamics of hot electrons. 
